Backdoor Secrets Unveiled: Identifying Backdoor Data with Optimized Scaled Prediction Consistency

Modern machine learning (ML) systems demand substantial training data, often resorting to external sources. Nevertheless, this practice renders them vulnerable to backdoor poisoning attacks. Prior backdoor defense strategies have primarily focused on the identification of backdoored models or poisoned data characteristics, typically operating under the assumption of access to clean data. In this work, we delve into a relatively underexplored challenge: the automatic identification of backdoor data within a poisoned dataset, all under realistic conditions, i.e., without the need for additional clean data or without manually defining a threshold for backdoor detection. We draw an inspiration from the scaled prediction consistency (SPC) technique, which exploits the prediction invariance of poisoned data to an input scaling factor. Based on this, we pose the backdoor data identification problem as a hierarchical data splitting optimization problem, leveraging a novel SPC-based loss function as the primary optimization objective. Our innovation unfolds in several key aspects. First, we revisit the vanilla SPC method, unveiling its limitations in addressing the proposed backdoor identification problem. Subsequently, we develop a bi-level optimization-based approach to precisely identify backdoor data by minimizing the advanced SPC loss. Finally, we demonstrate the efficacy of our proposal against a spectrum of backdoor attacks, encompassing basic label-corrupted attacks as well as more sophisticated clean-label attacks, evaluated across various benchmark datasets. Experiment results show that our approach often surpasses the performance of current baselines in identifying backdoor data points, resulting in about 4%-36% improvement in average AUROC. Codes are available at https://github.com/OPTML-Group/BackdoorMSPC.

==> sections/beneficialmaskfig.tex <==
\begin{figure}[t]
% \vspace*{-5mm}
%\vspace*{-6mm}
\centerline{
\includegraphics[width=\textwidth,height=!]{figs/Maskbenefit.pdf}
}
%\vspace*{-3.3mm}
\caption{\footnotesize{Benefit of Masks Imagenet
}}
  \label{fig: maskbenefit}
 % \vspace*{-4mm}
\end{figure}%%%


==> sections/bilevel.tex <==
\paragraph{Backdoor Identification via bi-level optimization.}
% We propose a hierarchical data-splitting optimization method, which is a cornerstone of our work and provides a solution to \textit{(1)} \RW{You can use \noindent\ding{182}} Finding $\mathbf{m} $ for \ref{eq: MSPC} \RW{use eqref instead of ref for equations}. \textit{(2)} satisfy both constraints \textbf{P1} and \textbf{P2}.
% Thus allows us to fully utilize the potential of the proposed MSPC loss and   draws from the insights in \citep{zeng2022sift}. 
% \RW{rewrite: We suggest a hierarchical method for optimizing data-splitting, serving as a fundamental element of our research, offering a solution to find $\mathbf{m}$ in alignment with \eqref{eq: MSPC} and satisfying both constraints \textbf{P1} and \textbf{P2}. This approach enables us to maximize the potential of the proposed MSPC loss, incorporating insights from \citep{zeng2022sift}.}
We propose a hierarchical data-splitting optimization method, serving as a fundamental element of our research, offering a solution to find $\mathbf{m}$ in alignment with \eqref{eq: MSPC} and satisfying both constraints \textbf{P1} and \textbf{P2}. This approach enables us to maximize the potential of the proposed MSPC loss, incorporating insights from \citep{zeng2022sift}.

We consider the following 



Recall that the vanilla data sifting problem was defined by   \eqref{eq: SPC} if the proper backdoor learning loss $L$ exists, and  it can be easily solved through some thresholding operations. However,  such a solution does not work for our proposed MSPC loss because we are not aware of a mask that focuses on the  `effective part' of a trigger. To address this, the data splitting problem of   \eqref{eq: Eq1} can be modified and  formulated  in the form of   bi-level optimization as follows:

\vspace*{-5mm}
{\small{
\begin{align}
\begin{array}{ll}
    \displaystyle  \min_{\mathbf w \in \{0,1\}^N}  & \sum_{i=1}^N (1-w_i) \ L(\mathbf x_i, \boldsymbol \mu^*(\mathbf{w}))  \\
     \st  & \boldsymbol{\mu}^*(\mathbf{w}) = \argmax_{\boldsymbol \mu} \ \frac{1}{N}\sum_{i=1}^N w_i \ L(\mathbf x_i, \boldsymbol \mu)
\end{array}
% \displaystyle & \min_{\mathbf w \in \{0,1\}^N}  \sum_{i=1}^N (1-w_i) \ L(\mathbf x_i, \gamma^*(\mathbf{w})) \
%  \st  \ \gamma^*(\mathbf{w}) = \argmax_{\gamma} \ \frac{1}{N}\sum_{i=1}^N w_i \ L(\mathbf x_i, \gamma(\mathbf{w}))
    \label{eq: Eq1_v2}
\end{align}}}%
% \SL{[notation issue for $\mathbf x_i$?]}

In \eqref{eq: Eq1_v2}, we regard the loss parameters $\boldsymbol{\mu}$ (\textit{e.g.}, masking variable $\mathbf{m}$ in MSPC) as another optimization variable for a newly introduced \textit{lower-level} optimization problem. In addition, the original SPC optimization is considered for an \textit{upper-level} problem that involves the lower-level solution $\boldsymbol{\mu}^(\mathbf w)$, which is also a function of the upper-level variables $\mathbf w$.
Given the generic bi-level form in \eqref{eq: Eq1_v2},
both the upper and lower level optimizations work cohesively towards distinguishing between the backdoor samples and the clean ones. The lower level optimization tackles this challenge by amplifying the representation of backdoor samples within the loss.
% \SL{loss? parameter?}\SP{changed} $L$. 
Conversely, the upper level optimization seeks to achieve the same goal by reducing the contribution of the poisoned samples within $L$. We note that this framework is different from bi-level optimization used for sifting out clean samples in  \cite{zeng2022sift}, where $L$ is simply the cross entropy loss and $\boldsymbol{\mu}$ represents the parameters of a neural network model. %\RW{We need to be careful here. Any other differences other than the loss type?} \RW{$\gamma$ is unclear for readers without any background. (1) Does $\gamma$ represent $m$ and $\theta$ and $\mathbf w$? (2) Why does the lower level $\gamma$ also has a $\star$ and why does it relate to $\mathbf w$?}

We next need to integrate our proposed MSPC loss   with the bi-level framework \eqref{eq: Eq1_v2}.
% Similar to the purpose of \eqref{eq: Eq1}, one can use our proposed MSPC loss to distinguish between poisoned and clean samples. 
 However, the MSPC loss is non-differentiable because of the occurrence of the function $\phi(x)$. We will now describe the strategies we adopt in each optimization level, to mitigate such issues, leading to our proposed bi-level solution.
 % next delve into the specifics of each level of the bi-level optimization formulation and explore strategies to circumvent such challenges. 
 % \SL{[rewrite this sentence, difficult to digest.]}\SP{Please check}

\RW{Do we need two separate paragraphs to discuss lower and upper-level optimization? We can save some space by just incorporating key parts under the bi-level optimization.}
\SL{[Yes, we do not need two extra subsections.]}


%\textbf{Lower-level optimization of \eqref{eq: Eq1_v2}.} 
% \SL{[notation issues in the following. Please carefully check and revise this part. \textit{e.g.}, $\mathbf n$ or $n$? $\mathbf m$ or $m$? ]}
% In Section \ref{sec: SPCRevisit}, we developed insights as to how the use of masks can alleviate some of the issues of the SPC loss.Moreover, this naturally creates the desired parameterization of the SPC loss: $\ell_{SPC} (\mathbf{x}, m) = \ell_{SPC} (\mathbf{x}^m_i)$.
First, the basis of the scaled prediction consistency is that for poisoned samples, the predicted class of a model for an input $\mathbf{x}$ remains consistent even when multiplied with scales, \textit{i.e.}, $\argmax\mathcal{F}_{\boldsymbol \theta}(\cdot)$ remains the same. Thus, for a sample $\mathbf{x}_i$ and for a scale $n \in \mathcal{S}$, maximizing the SPC loss would result in maximizing a non-differentiable loss $\mathbbm{1}(\displaystyle \argmax\mathcal{F}_{\boldsymbol \theta}(\mathbf{x}) = \displaystyle \argmax\mathcal{F}_{\boldsymbol \theta}(n\cdot\mathbf{x}))$ for SPC or maximizing the non-differentiable $\phi(\displaystyle \argmax\mathcal{F}_{\boldsymbol \theta}(\mathbf{x}) - \displaystyle \argmax\mathcal{F}_{\boldsymbol \theta}(n\cdot\mathbf{x}))$ for the MSPC loss. In such a scenario, we argue that the probability distribution that we get from the model for poisoned inputs across scales would also remain similar, \textit{i.e.}, the distance between $\mathcal{F}_{\boldsymbol \theta}(\mathbf{x})$ and $\mathcal{F}_{\boldsymbol \theta}(n\cdot \mathbf{x})$ would remain small when $\mathbf{x} \in \mathcal{D}_b$.  Based on that, we can simply replace the non-differentiable loss maximization with the minimization of the Kullback-Leibler (KL) divergence. Specifically, this involves minimizing the divergence between the probability distribution output for a sample $\mathbf{x}_i$ and the output for the same sample when masked with $\mathbf{m}$ and subsequently scaled with $n$. This is in line with our proposed use of masks $\mathbf{m}$. In mathematical terms, this is denoted as $\min_{\mathbf{m}} D_{KL} (\mathcal{F}_{\boldsymbol \theta}(\mathbf{x}_i) || \mathcal{F}_{\boldsymbol \theta}(n \cdot\mathbf{x}_i^\mathbf{m}))$. Moreover, since our mask $\mathbf{m}$ focuses on the `effective part' of the trigger, we also penalize the size of the mask similar to \citep{huang2023distilling}.  
Leveraging the advantages of the proposed linear shift by $\tau$, we can customize the \textbf{lower-level optimization} of \eqref{eq: Eq1_v2}  to
% \vspace*{0.1mm}

\vspace*{-3mm}
{\small{
\begin{align}
 \mathbf{m}^*(\mathbf w) = \argmin_{\mathbf{m}} \ \frac{1}{N}\sum_{i=1}^N  \Big[ w_i\ \frac{1}{|S|}\sum_{n \in S} D_{KL} (\mathcal{F}_{\boldsymbol \theta}(\mathbf{x}_i) || \mathcal{F}_{\boldsymbol \theta}(n \cdot\mathbf{x}_i^{m}))\Big] + \lambda \|\mathbf{m}\|_1 , 
    \label{eq: Eq2}
\end{align}}}%
where recall that $\mathbf{x}_i^{m} = (\mathbf{x}_i - \tau) \odot \mathbf{m}$.
The above addresses the challenge of optimizing the mask variable in a non-differentiable loss function by converting the lower-level optimization to a differentiable one,   achieved through utilizing KL divergence. 

% \RW{Why don't we add and discuss $\lambda \|\mathbf{m}\|_1$ here?}

% \SL{[notation issues: $\mathbf x_i$ rather than $\mathbf{x}_i$. Also, $\mathbf x_i^m$ instead of $\mathbf{x}_i^m $? Please check the above very very carefully!]}

%\textbf{Upper-level optimization of \eqref{eq: Eq1_v2}.} 

 
 For the \textbf{upper-level optimization}, we propose the direct use of the MSPC loss. 
Thus, we finally achieve our proposed bi-level optimization problem: 
% \RW{we should use a different notation in $\mathbf{m}^*(\mathbf{w})$ in the upper optimization or at least mention that we relax the optimization to only consider the w outside of the NSPC loss term} 
% \SL{What is MSPC? This advancement should be defined separately \textit{e.g.}, assuming $\mathbf m$ is known a prior. Then this section tries to relax this assumption!}


\vspace*{-5mm}
{\small{
\begin{align}
\begin{array}{ll}
\displaystyle  \min_{\mathbf w \in [0,1]^N}  &\sum_{i=1}^N (1-w_i) \ \ell_\mathrm{MSPC} (\mathbf{x}_i, \mathbf{m}^*(\mathbf{w}),  \tau)
  %\Big\langle (1-{\mathbf w}), l_{MSPC} (\mathbf{x} \odot \mathbf{m}^*(\mathbf{w}); \btheta) \Big\rangle 
  \\
 \st  & \text{$\mathbf{m}^*(\mathbf{w})$ is obtained by \eqref{eq: Eq2},}
 % \ \mathbf{m}^*(\mathbf{w}) = \argmin_{\mathbf m \in [0,1]^{\mathrm{H} \times \mathrm{W}}} \ \frac{1}{N}\sum_{i=1}^N \Big[ w_i\ \frac{1}{|S|}\sum_{n \in S} D_{KL} (\mathcal{F}_{\boldsymbol \theta}(\mathbf{x}_i) || \mathcal{F}_{\boldsymbol \theta}(n.\mathbf{x}_i^m))\Big] + \lambda \|\mathbf{m}\|_1, 
\end{array}
\label{eq: bilevel}
\end{align}
}}%
% where consider the image height and width to be $\mathrm{H}$ and $\mathrm{W}$ respectively.
% \SL{[I did not understand the last sentence. Remove or re-write it.] \SP{m is constrained between 0 and 1. Hence I added that part}}

We note that the upper level is intricately linked with the lower level optimization, rendering the problem more complex. In practical terms, we managed to simplify this by treating the $\mathbf{m}^*(\mathbf{w})$ term in the upper optimization as a given value, considering only the $\mathbf w$ variable outside the MSPC loss. In this way, we can still use the MSPC loss in the upper-level optimization. The resulting approach is known as   alternating optimization   for solving bi-level problems \citep{liu2021investigating}.
%as we do not need to directly calculate the gradient of the MSPC loss. 
This approach, although a compromise, yielded satisfactory results and significantly reduced the complexity of our optimization process.
% \SL{where xxxx, [missing $\ell_1 $ regularization explanation? Please carefully check your notations as well! $\mathbf m$?]}
Moreover, we relax  $\mathbf{w}$ to lie between 0 and 1 for ease of solving by converting a potential combinatorial optimization problem to a continuous one.

Thus we solve this bi-level optimization problem in \eqref{eq: bilevel} by using simple alternating optimization, starting from the upper level.  Specifically, we initialize the mask with the value of 1 for all pixels. We note that minimizing the upper level optimization is trivial in our case: we set $w_i = 1$ if $\ell_\mathrm{MSPC} (\mathbf{x}_i, \mathbf{m} ,\tau)$ is positive and $w_i = 0$ if $\ell_\mathrm{MSPC} (\mathbf{x}_i, \mathbf{m} ,\tau)$ is negative. We choose an odd number of scales for our experiments so that the value of the MSPC loss is never 0. During this upper level optimization we consider the mask $\mathbf{m(w)}$ to be fixed. Solving the upper level optimization yields us a $\mathbf{w}$, which we use to solve the lower level optimization using gradient descent. We can perform this process iteratively to find the final MSPC loss vector where the $i$th value of this vector is given by $\ell_\mathrm{MSPC} (\mathbf{x}_i, \mathbf{m}^*(\mathbf{w}^*),  \tau)$. We calculate the AUROC in Section \ref{sec: Exp} \SL{[Check this. Typo.]} using this MSPC loss vector. Moreover, because of \eqref{eq: MSPC}, we can simply threshold the vector at 0, to sift the backdoor samples with MSPC loss values greater than 1.


==> sections/ncrfig.tex <==
\begin{wrapfigure}{r}{55mm}
% \vspace*{-17mm}
\vspace*{-5mm}
\centerline{
\includegraphics[width=55mm,height=!]{figs/NCR.pdf}
}
\vspace*{-3mm}
\caption{\footnotesize{Normalized Corruption Ratio for different percentages of clean samples sifted out. If $\mathbf x$ clean samples are identified, NCR = ((number of poison samples in $\mathbf x$) / $\mathbf x$) \ / poison ratio $\times 100 \%$.
}}
  \label{fig: ncr}
 % \vspace*{-7mm}
\end{wrapfigure}%%%

==> sections/tableretrain.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\vspace{-3mm}
\centering
\caption{\footnotesize{
Effect of retraining models without backdoor samples identified by our algorithm. ACC denotes standard accuracy, ASR denotes the Attack Success Rate.
} 
}
\label{tab: retrain}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule[1pt]
\midrule
\multirow{2}{*}{Attack} & \multicolumn{2}{c}{Before} & \multicolumn{2}{c}{After} \\
& ACC & ASR & ACC & ASR \\
\rowcolor{LightCyan}
\midrule
\multicolumn{5}{c}{\textbf{CIFAR10}} \\
\midrule
Badnet & 88.36 (0.12) & 100.00 (0.00) &81.35 (0.89) & 0.52 (0.60) \\ 
Blend & 88.29 (0.32) & 100.00 (0.00) &79.28 (0.89) & 3.85 (5.45) \\ 
LabelConsistent & 89.36 (0.42) & 99.31 (0.33) &83.08 (1.38) & 2.59 (3.62) \\ 
Trojan & 88.62 (0.09) & 100.00 (0.00) &79.58 (0.71) & 0.00 (0.00) \\ 
Wanet & 88.20 (0.20) & 98.53 (0.18) &79.40 (1.06) & 32.94 (46.59) \\ 
 \rowcolor{LightCyan}
\midrule
\multicolumn{5}{c}{\textbf{Tiny Imagenet}} \\
\midrule
Badnet & 53.04 (0.53) & 99.24 (0.20) &54.09 (0.20) & 0.14 (0.06) \\ 
Blend & 53.16 (0.26) & 99.84 (0.04) &53.55 (0.26) & 32.41 (32.06) \\ 
\rowcolor{LightCyan}
\midrule
\multicolumn{5}{c}{\textbf{Imagenet200}} \\
\midrule
Badnet & 62.43 (0.29) & 99.99 (0.00) &62.39 (0.18) & 0.08 (0.03) \\ 
Blend & 62.04 (0.18) & 99.61 (0.04) &62.61 (0.13) & 89.29 (1.58) \\
\midrule
\bottomrule[1pt]
\end{tabular}
}
\end{wraptable}
% \end{table*}
% \begin{table}
% \centering
% \caption{\footnotesize{
% Effect of retraining models without backdoor samples identified by our algorithm. ACC denotes standard accuracy , ASR denotes the Attack Success Rate, where  the standard deviation is given in parenthesis, and the values of mean and standard deviation are calculated over 3 runs.
% } 
% }
% \label{tab: retrain}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c}
% \toprule[1pt]
% \midrule
% \multirow{2}{*}{Attack} & \multicolumn{2}{c}{Before} & \multicolumn{2}{c}{After} \\
% & ACC & ASR & ACC & ASR \\
% \rowcolor{LightCyan}
% \midrule
% \multicolumn{5}{c}{\textbf{CIFAR10}} \\
% \midrule
% Badnet & 88.36 (0.12) & 100.00 (0.00) &81.35 (0.89) & 0.52 (0.60) \\ 
% Blend & 88.29 (0.32) & 100.00 (0.00) &79.28 (0.89) & 3.85 (5.45) \\ 
% LabelConsistent & 89.36 (0.42) & 99.31 (0.33) &83.08 (1.38) & 2.59 (3.62) \\ 
% Trojan & 88.62 (0.09) & 100.00 (0.00) &79.58 (0.71) & 0.00 (0.00) \\ 
% Wanet & 88.20 (0.20) & 98.53 (0.18) &79.40 (1.06) & 32.94 (46.59) \\ 
%  \rowcolor{LightCyan}
% \midrule
% \multicolumn{5}{c}{\textbf{Tiny Imagenet}} \\
% \midrule
% Badnet & 53.04 (0.53) & 99.24 (0.20) &54.09 (0.20) & 0.14 (0.06) \\ 
% Blend & 53.16 (0.26) & 99.84 (0.04) &53.55 (0.26) & 32.41 (32.06) \\ 
% \rowcolor{LightCyan}
% \midrule
% \multicolumn{5}{c}{\textbf{Imagenet200}} \\
% \midrule
% Badnet & 62.43 (0.29) & 99.99 (0.00) &62.39 (0.18) & 0.08 (0.03) \\ 
% Blend & 62.04 (0.18) & 99.61 (0.04) &62.61 (0.13) & 89.29 (1.58) \\
% \midrule
% \bottomrule[1pt]
% \end{tabular}
% }
% \end{table}


==> sections/uniquemaskfig.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
% \vspace*{-5mm}
%\vspace*{-6mm}
\centerline{
\includegraphics[width=0.5\textwidth,height=!]{figs/Maskunique.pdf}
}
%\vspace*{-3.3mm}
\caption{\footnotesize{Unique Masks CIFAR10
}}
  \label{fig: visual_mask}
 \vspace*{-3mm}
\end{wrapfigure}%%%

